Enabling Efficient Hybrid Systolic Computation in Shared L1-Memory Manycore Clusters

Systolic arrays and shared-L1-memory manycore clusters are commonly used architectural paradigms that offer different trade-offs to accelerate parallel workloads. While the first excel with regular dataflow at the cost of rigid architectures and complex programming models, the second are versatile and easy to program but require explicit dataflow management and synchronization. This work aims at enabling efficient systolic execution on shared-L1-memory manycore clusters. We devise a flexible architecture where small and energy-efficient RISC-V cores act as the systolic array's processing elements (PEs) and can form diverse, reconfigurable systolic topologies through queues mapped in the cluster's shared memory. We introduce two low-overhead RISC-V ISA extensions for efficient systolic execution, namely Xqueue and Queue-linked registers (QLRs), which support queue management in hardware. The Xqueue extension enables single-instruction access to shared-memory-mapped queues, while QLRs allow implicit and autonomous access to them, relieving the cores of explicit communication instructions. We demonstrate Xqueue and QLRs in MemPool, an open-source shared-memory cluster with 256 PEs, and analyze the hybrid systolic-shared-memory architecture's trade-offs on several DSP kernels with diverse arithmetic intensity. For an area increase of just 6%, our hybrid architecture can double MemPool's compute unit utilization, reaching up to 73%. In typical conditions (TT/0.80V/25{\deg}C), in a 22 nm FDX technology, our hybrid architecture runs at 600 MHz with no frequency degradation and is up to 65% more energy efficient than the shared-memory baseline, achieving up to 208 GOPS/W, with up to 63% of power spent in the PEs.

==> Makefile <==
LATEXMK := latexmk -quiet -pdf -bibtex

tex_target := main

figs_obj = $(wildcard fig/*.obj)
figs_eps = $(wildcard fig/*.eps)
figs_svg = $(wildcard fig/*.svg)
figs_tex = $(wildcard fig/*.tex)

figs_obj_pdf = $(patsubst %.obj,%.pdf,$(figs_obj))
figs_eps_pdf = $(patsubst %.eps,%.pdf,$(figs_eps))
figs_svg_pdf = $(patsubst %.svg,%.pdf,$(figs_svg))
figs_tex_pdf = $(patsubst %.tex,%.pdf,$(figs_tex))
figs_pdf = $(figs_obj_pdf) $(figs_eps_pdf) $(figs_svg_pdf) $(figs_tex_pdf)

.PHONY: all
all: $(tex_target).pdf

# Declare the PDF output file as phony because we do not want to rely on Make's dependency
# resolution (getting it to work properly with LaTeX is very difficult).  Instead, we always invoke
# `latexmk` and let that tool decide which steps to take (it was designed for this task).
.PHONY: $(tex_target).pdf
$(tex_target).pdf: $(figs_pdf)
	$(LATEXMK) $(tex_target).tex

.PHONY: $(tex_target).txt
$(tex_target).txt:
	pandoc --from=latex --to=plain --wrap=none $(tex_target).tex > $@

tmpdir := $(shell mktemp -d)
$(tex_target).tar.gz: $(tex_target).pdf dist-clean
	mkdir $(tmpdir)/$(tex_target)
	rsync -a --exclude='.git/' --exclude='$@' . $(tmpdir)/$(tex_target)
	tar czf $@ -C $(tmpdir) $(tex_target)
	rm -r $(tmpdir)

$(figs_obj_pdf): %.pdf : %.obj
	tgif -print -eps -color $*.obj
	epstopdf $*.eps
	rm $*.eps

$(figs_eps_pdf): %.pdf : %.eps
	epstopdf $*.eps

$(figs_svg_pdf): %.pdf : %.svg
	inkscape --without-gui --export-pdf=$*.pdf $*.svg

$(figs_tex_pdf): %.pdf : %.tex
	$(LATEXMK) -cd $*.tex

.PHONY: live
live::
	$(LATEXMK) -pvc $(tex_target).tex

.PHONY: stats
stats:
	$(LATEXMK) -jobname=full -pdflatex="pdflatex %O '\input{%S}'" $(tex_target).tex
	$(LATEXMK) -jobname=nooutline -pdflatex="pdflatex %O '\newcommand{\outline}[1]{}\input{%S}'" $(tex_target).tex
	$(LATEXMK) -jobname=notodo -pdflatex="pdflatex %O '\newcommand{\todo}[1]{}\input{%S}'" $(tex_target).tex
	full=$$(pdftotext build/full.pdf - | wc -w); \
	nooutline=$$(pdftotext build/nooutline.pdf - | wc -w); \
	notodo=$$(pdftotext build/notodo.pdf - | wc -w); \
	echo "Todo   : $$(( $${full}-$${notodo}))"; \
	echo "Outline: $$(( $${full}-$${nooutline}))"; \
	echo "Text   : $$(( -$${full}+$${notodo}+$${nooutline}))"

.PHONY: clean
clean:: clean-figs
	latexmk -C -bibtex
	rm -f $(tex_target).tar.gz

.PHONY: clean-figs
clean-figs:
	rm -f $(figs_pdf)

.PHONY: dist-clean
dist-clean::
	latexmk -c

